AutoSlicer: Scalable Automated Data Slicing for ML Model Analysis

Automated slicing aims to identify subsets of evaluation data where a trained model performs anomalously. This is an important problem for machine learning pipelines in production since it plays a key role in model debugging and comparison, as well as the diagnosis of fairness issues. Scalability has become a critical requirement for any automated slicing system due to the large search space of possible slices and the growing scale of data. We present Autoslicer, a scalable system that searches for problematic slices through distributed metric computation and hypothesis testing. We develop an efficient strategy that reduces the search space through pruning and prioritization. In the experiments, we show that our search strategy finds most of the anomalous slices by inspecting a small portion of the search space.

==> figures/priority_example.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.96\linewidth]{figures/priority_example.eps}
    \caption{An illustration of the priority queue-based strategy when the $p$-value threshold is set to $0.05$. $P_1, P_2, P_3, P_4$ are singleton predicates, and the numbers following them represent the $p$-values of the corresponding slices. After the first iteration, all slices with singleton predicates have been computed. $S_{P_1}$ is significant so we prune all of its children based on the early stopping criterion. $S_{P_2}$ has the lowest $p$-value and thus the highest priority. Therefore, only $S_{P_2}$ is subdivided in the next iteration if the limit for the number of candidate slices is $2$.}
    \label{fig:priority_example}
\end{figure*}

==> tables/runtimeManagement.tex <==
\begin{table}[t]
\caption{Experiments in the runtime-bounded mode.}
\vspace{-2mm}
\center
\label{tab:runtime_bounded}
\small
\begin{tabular}{lccccc}
\toprule
Dataset & \thead{\small{Time Limit} \\ \small{(min)}} & \thead{\small{Actual Runtime} \\ \small{(min)}} & \thead{\small{\# Iterations} \\ \small{Finished}}\\
\midrule
\multirow{3}{*}{OpenML Electricity} & 10 & 9 & 2\\
                                    & 20 & 14 & 5\\
                                    & 30 & 20 & 5\\
\midrule                                    
\multirow{3}{*}{Traffic Stop Fairness} & 90 & 74 & 5\\
                                    & 180 & 162 & 5\\
                                    & 270 & 232 & 5\\
\midrule
\multirow{3}{*}{UCI Census}         & 30 & 29 & 2\\
                                    & 60 & 68 & 1\\
                                    & 90 & 90 & 5\\
\bottomrule
\end{tabular}
\end{table}
